Role Prompting Guided Domain Adaptation with General Capability Preserve for Large Language Models

The growing interest in Large Language Models (LLMs) for specialized applications has revealed a significant challenge: when tailored to specific domains, LLMs tend to experience catastrophic forgetting, compromising their general capabilities and leading to a suboptimal user experience. Additionally, crafting a versatile model for multiple domains simultaneously often results in a decline in overall performance due to confusion between domains. In response to these issues, we present the RolE Prompting Guided Multi-Domain Adaptation (REGA) strategy. This novel approach effectively manages multi-domain LLM adaptation through three key components: 1) Self-Distillation constructs and replays general-domain exemplars to alleviate catastrophic forgetting. 2) Role Prompting assigns a central prompt to the general domain and a unique role prompt to each specific domain to minimize inter-domain confusion during training. 3) Role Integration reuses and integrates a small portion of domain-specific data to the general-domain data, which are trained under the guidance of the central prompt. The central prompt is used for a streamlined inference process, removing the necessity to switch prompts for different domains. Empirical results demonstrate that REGA effectively alleviates catastrophic forgetting and inter-domain confusion. This leads to improved domain-specific performance compared to standard fine-tuned models, while still preserving robust general capabilities.

==> cross_meta.tex <==
\begin{table*}[ht]
\centering
\small
\begin{tabular}{c|c|ccc|cc|cccccc}
\toprule
\multirow{2}{*}{Prompt} & \multicolumn{1}{c}{General} & \multicolumn{3}{c}{Medical} & \multicolumn{2}{c}{Law} & \multicolumn{6}{c}{Finance} \\

\cmidrule(lr){2-2}\cmidrule(lr){3-5}\cmidrule(lr){6-7}\cmidrule(lr){8-13}
  &GEv & QQ & TC & MQA & LQA & LS & FNA & FQA & FNL & FRE & FFE &FSP\\ 
\midrule

\rowcolor[rgb]{0.93,0.93,0.93}\multicolumn{13}{c}{\textit{BELLE-7B}} \\

Mix  & 6.26 & {85.21} & 74.44& 32.64 & 57.04& 44.29& 59.81&75.10 &91.31 &47.76 & {69.57} &85.44\\



{MEGA}$^g$   & \cellcolor{red!20}{6.87} & 82.39 & \cellcolor{red!20}{76.69} & \cellcolor{red!20}{37.95} &\cellcolor{red!20}57.65 & \cellcolor{red!20}{46.90}& \cellcolor{red!20}{61.68}&\cellcolor{red!20}{78.18} &\cellcolor{red!20}{95.65} &\cellcolor{red!20}{55.22} &68.48 & \cellcolor{red!20}{85.68} \\
\rowcolor{green!20}\multicolumn{13}{c}{\textit{MEGA with Different Area Prompts}} \\

{MEGA}$^m$   & 6.05& \cellcolor{red!20} 84.51 & \cellcolor{red!20} {78.20} & {37.45} & 56.05 & 44.38 & 61.09 & 69.31 & {94.77} & 53.15& 67.39 & 85.41\\

{MEGA}$^l$   & 6.11&82.39 & {75.93}& {36.24} &\cellcolor{red!20}{58.18}& 46.52&{61.42}& 73.52 &{94.43} &{53.61} & 68.32 & 84.03 \\

{MEGA}$^f$   & \cellcolor{red!20}{6.30} & \cellcolor{red!20}83.10 &{75.94} & {36.57}&{56.55} & 43.27 & 60.91& 77.26&{93.47} &{53.73} & \cellcolor{red!20}{70.65} & 85.37 \\

\midrule

\rowcolor[rgb]{0.93,0.93,0.93}\multicolumn{13}{c}{\textit{BELLE-13B}} \\

Mix & 6.92 & 84.37 & 78.95 & 36.47 & 58.43 & 44.58 & 61.67 & 74.69 & 93.48 & 59.29 & 72.83 & 77.76  \\



{MEGA}$^g$  & 7.75 & \cellcolor{red!20}{85.33} & \cellcolor{red!20}79.22 & \cellcolor{red!20}{37.67} & 58.11 & \cellcolor{red!20}{47.52} & \cellcolor{red!20}{62.27} & \cellcolor{red!20}{77.79} & 92.33& \cellcolor{red!20}{62.37}& \cellcolor{red!20}{73.71} & \cellcolor{red!20}{88.06}\\
\rowcolor{green!20}\multicolumn{13}{c}{\textit{MEGA with Different Area Prompts}} \\

{MEGA}$^m$ & 7.12 & \cellcolor{red!20}85.92 & \cellcolor{red!20}79.70 & \cellcolor{red!20}39.31 & 57.86 & 45.91 & 61.91 & 65.87 & 91.30 & 61.19 & 68.91 & 83.79\\

{MEGA}$^l$ & 7.33 &79.58 & 76.65 & \cellcolor{red!20}37.99 & \cellcolor{red!20}58.84 & 46.93 & 62.07 & 65.30 & 91.24 & 61.20 & 67.58 & 81.98 \\

{MEGA}$^f$ &7.54 & 78.17 & 76.71 & 37.76 &  57.54 & 43.86 & \cellcolor{red!20}62.55 & 68.62 & \cellcolor{red!20}92.47 & 61.73 & 69.57 & 80.62  \\

\bottomrule
\end{tabular}
\caption{Performance of BELLE-7B with different Meta-Prompts. Scores better than \textbf{Mix} are in red background.}
\label{tab:cross_test}
\end{table*}


% -------------------------------------

% \begin{table*}[ht]
% \centering
% \small
% \begin{tabular}{c|cc|ccc|cc|cccccc}
% \toprule
% \multirow{2}{*}{Prompt} & \multicolumn{2}{c}{General} & \multicolumn{3}{c}{Medical} & \multicolumn{2}{c}{Law} & \multicolumn{6}{c}{Finance} \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-6}\cmidrule(lr){7-8}\cmidrule(lr){9-14}
%  & CEval &GEv & QQ & TC & MQA & LQA & LS & FNA & FQA & FNL & FRE & FFE &FSP\\ 
% \midrule
% Mix & 27.71 & 6.67 & 85.21 & 74.44& 32.64 & 57.04& 44.29& 59.81&75.10 &97.83 &46.90 & 69.57 &85.44\\

% \rowcolor{green!20}\multicolumn{14}{c}{\textit{Meta Prompt}} \\

% General & \cellcolor{red!20}{28.68} & \cellcolor{red!10}6.82 & \cellcolor{blue!15}82.39 & \cellcolor{red!10}{76.69} & \cellcolor{red!20}{37.52} & \cellcolor{blue!10}56.65 & \cellcolor{red!10}{45.15}& \cellcolor{red!20}{61.51}& \cellcolor{red!10}{78.16} & \cellcolor{red!20}{98.79} & \cellcolor{red!20}{59.36} & \cellcolor{blue!10}68.48 & \cellcolor{red!10}{85.68}\\

% Med & \cellcolor{blue!10}27.19 & 6.05& \cellcolor{blue!10}84.51 & \cellcolor{red!20}78.20 & \cellcolor{red!20}37.45 & \cellcolor{red!10}57.78 & \cellcolor{blue!10}39.48 & \cellcolor{red!10}61.20 & \cellcolor{blue!10}69.31 & \cellcolor{red!10}98.31 & \cellcolor{red!10}53.87& \cellcolor{blue!20}66.30& \cellcolor{blue!10}84.19\\

% Law & \cellcolor{red!10}27.78 & 6.11& \cellcolor{red!5}85.21 & \cellcolor{red!10}75.93& \cellcolor{red!20}36.24 & \cellcolor{red!10}57.56& \cellcolor{blue!10}40.50& \cellcolor{red!20}61.66& \cellcolor{blue!20}67.99 &\cellcolor{red!20}98.79 &\cellcolor{red!10}53.98 & \cellcolor{blue!10}68.48 & \cellcolor{blue!10}84.03\\

% Fin & \cellcolor{blue!10}27.04 & 6.30& \cellcolor{blue!15}83.10 & \cellcolor{red!20}77.44 & \cellcolor{red!20}36.64& \cellcolor{red!10}57.46 & \cellcolor{blue!10}40.63 & \cellcolor{red!10}60.91& \cellcolor{blue!20}68.78& \cellcolor{red!20}98.79 &\cellcolor{red!10}53.58 & \cellcolor{red!5}69.57 & \cellcolor{blue!10}84.39 \\

% \bottomrule
% \end{tabular}
% \caption{Performance of BELLE-7B with different meta-prompts. Mix-rate \~9\%}
% \label{tab:cross_test}
% \end{table*}

==> en_mix_rate.tex <==
\begin{table}[ht]
\centering
\small
\begin{tabular}{c|cc|ccc}
\toprule
 \multirow{2}{*}{Model}  & \multicolumn{2}{c}{General} & \multicolumn{3}{c}{Medical}  \\
\cmidrule(lr){2-3}\cmidrule(lr){4-6} 
& CEval & GEv & QQ & TC & MQA \\ 
\midrule
BELLE &25.60 &7.42 & 8.80 & 1.60 & 36.32\\
\rowcolor[rgb]{0.93,0.93,0.93}\multicolumn{6}{c}{\textit{LoRA}} \\
+FT & & 5.52 & 84.40 & 75.80 & 34.15\\
+Mix & & 6.55 & 83.80 & 73.40 & 33.05\\
+MMix & & 6.82 & 83.00 & 74.60 & 34.97\\

\bottomrule
\end{tabular}
\caption{Performance of Belle-7B on Medical.}
\label{tab:zh_mix_rate}
\end{table}

==> eng_FTAP.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{c|c|cc|c|c}
\toprule
\multirow{2}{*}{Model} & \multicolumn{1}{c}{General} & \multicolumn{2}{c}{Medical} & \multicolumn{1}{c}{Law} & \multicolumn{1}{c}{Finance} \\
\cmidrule(lr){2-2}\cmidrule(lr){3-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}
 & MTBc & PMQA & MMQA & CHQA & FBQA \\ 
\midrule
\rowcolor[rgb]{0.93,0.93,0.93}\multicolumn{6}{c}{\textit{Vicuna2-7B}} \\

FT & & 52.17 & 42.07 & 66.80 & 32.17\\
Mix & & 60.87 & {42.27} & 67.20 & 39.12\\
\rowcolor{green!20}\multicolumn{6}{c}{\textit{FTAP with Different Area Prompts}} \\
 {FTAP}$^m$   & & \textbf{65.22} & 41.12 & 64.20 & 53.58 \\
 {FTAP}$^l$   & & 64.89 & 38.99 & \textbf{68.12} & 54.47 \\
 {FTAP}$^f$   & & 63.39 & 38.11 & 60.40 & \textbf{55.12}\\
\bottomrule
\end{tabular}
\caption{Performance of vicuna-7B-FTAP.}
\label{tab:english_FTAP}
\end{table}

==> zh_FTAP.tex <==
\begin{table*}[ht]
\centering
\small
\begin{tabular}{c|c|ccc|cc|cccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{1}{c}{General} & \multicolumn{3}{c}{Medical} & \multicolumn{2}{c}{Law} & \multicolumn{6}{c}{Finance} \\
\cmidrule(lr){2-2}\cmidrule(lr){3-5}\cmidrule(lr){6-7}\cmidrule(lr){8-13}
  & GEv & QQ & TC & MQA & LQA & LS & FNA & FQA & FNL & FRE & FFE &FSP\\ 
\midrule


FT  & 5.41 & 83.10 & 75.94 & 36.84 &\textbf{58.05} &44.82 &61.07 &72.83 & 93.47& 50.75& 67.39& 85.41\\
Mix  & 6.26 & \textbf{85.21} & 74.44& 32.64 & 57.04& 44.29& 59.81&75.10 &91.31 &47.76 & \textbf{69.57} &85.44\\
\rowcolor{green!20}\multicolumn{13}{c}{\textit{FTAP with Different Area Prompts}} \\
FTAP$^m$ & 5.55& 82.39 & \textbf{78.95} & \textbf{37.16} & 54.68 & 40.84 & 61.84 &80.47 &93.48 & 53.73 & 64.13 & 83.78 \\
FTAP$^l$ &5.67 & 81.52 & \textbf{76.69} & 36.68& 57.08 & \textbf{45.04} & 60.57 & \textbf{74.57} & 92.33 & 50.75 & 66.30 & 84.51 \\
FTAP$^f$ & 5.53& 81.37
& \textbf{76.22} & 34.32 & 54.76 & 36.33 & 61.02 & \textbf{80.53} & \textbf{93.48} & \textbf{55.22} & \textbf{71.74} & \textbf{85.68} \\

\bottomrule
\end{tabular}
\caption{Performance of BELLE
under different settings. Best scores are in \textbf{bold}.}
\label{tab:Chinese_performance}
\end{table*}

